ReEx-SQL: Reasoning with Execution-Aware Reinforcement Learning for Text-to-SQL

In Text-to-SQL, execution feedback is essential for guiding large language models (LLMs) to reason accurately and generate reliable SQL queries. However, existing methods treat execution feedback solely as a post-hoc signal for correction or selection, failing to integrate it into the generation process. This limitation hinders their ability to address reasoning errors as they occur, ultimately reducing query accuracy and robustness. To address this issue, we propose ReEx-SQL (Reasoning with Execution-Aware Reinforcement Learning), a framework for Text-to-SQL that enables models to interact with the database during decoding and dynamically adjust their reasoning based on execution feedback. ReEx-SQL introduces an execution-aware reasoning paradigm that interleaves intermediate SQL execution into reasoning paths, facilitating context-sensitive revisions. It achieves this through structured prompts with markup tags and a stepwise rollout strategy that integrates execution feedback into each stage of generation. To supervise policy learning, we develop a composite reward function that includes an exploration reward, explicitly encouraging effective database interaction. Additionally, ReEx-SQL adopts a tree-based decoding strategy to support exploratory reasoning, enabling dynamic expansion of alternative reasoning paths. Notably, ReEx-SQL achieves 88.8% on Spider and 64.9% on BIRD at the 7B scale, surpassing the standard reasoning baseline by 2.7% and 2.6%, respectively. It also shows robustness, achieving 85.2% on Spider-Realistic with leading performance. In addition, its tree-structured decoding improves efficiency and performance over linear decoding, reducing inference time by 51.9% on the BIRD development set.

==> sections/exp.tex <==

\section{Experiments}
\subsection{Experimental Settings}
%% Experimental Settings 包括 dataset， Metrics Implementation Details
%%% baseline 就不写了。
% \paragraph{Datasets and Metrics}
% We conduct experiments on two widely used Text-to-SQL benchmarks: BIRD~\citep{DBLP:conf/nips/bird} and Spider~\citep{DBLP:conf/emnlp/spider}. BIRD is a large-scale cross-domain dataset with over 12,000 queries across 95 databases from 37 professional domains, designed to better reflect real-world scenarios. We evaluate it using the official metrics: execution accuracy (EX) and valid efficiency score (VES), where VES measures the runtime efficiency of the predicted SQL relative to the ground truth. Spider covers 200 databases across 138 domains and serves as the standard benchmark for cross-domain generalization. For Spider and its three robustness variants—Spider-Syn~\citep{DBLP:conf/acl/Spider-Syn}, Spider-Realistic~\citep{DBLP:conf/naacl/Spider-Realistic}, and Spider-DK~\citep{DBLP:conf/emnlp/Spider-DK}—We follow the official evaluation protocol using execution accuracy (EX) and test-suite accuracy (TS)~\citep{Test-Suites}, where TS evaluates whether a SQL query produces correct results across multiple test cases in a test suite of databases, which are augmented with additional entries to ensure broader coverage.  Specifically, Spider-Syn replaces schema-related words with synonyms, Spider-Realistic removes explicitly mentioned column names from the questions, and Spider-DK introduces domain knowledge to rephrase the questions.
\paragraph{Datasets and Metrics}
We conduct experiments on two widely used Text-to-SQL benchmarks: BIRD~\citep{DBLP:conf/nips/bird} and Spider~\citep{DBLP:conf/emnlp/spider}. BIRD is a large-scale cross-domain dataset comprising over 12,000 queries across 95 databases spanning 37 professional domains, designed to better reflect real-world scenarios. It is evaluated using the official metrics: execution accuracy (EX) and valid efficiency score (VES), where VES measures the runtime efficiency of the predicted SQL compared to the ground truth. Spider, the standard benchmark for cross-domain generalization, includes 200 databases across 138 domains. In addition to Spider, we evaluate three of its robustness variants—Spider-Syn~\citep{DBLP:conf/acl/Spider-Syn}, Spider-Realistic~\citep{DBLP:conf/naacl/Spider-Realistic}, and Spider-DK~\citep{DBLP:conf/emnlp/Spider-DK}—following the official evaluation protocol. For Spider and its variants, we use execution accuracy (EX) and test-suite accuracy (TS)~\citep{Test-Suites}. TS assesses whether a SQL query produces correct results across multiple test cases in a test suite of databases, with augmented test suite of database entries ensuring broader coverage. Specifically, Spider-Syn replaces schema-related words with synonyms, Spider-Realistic removes explicitly mentioned column names from the questions, and Spider-DK incorporates domain knowledge to rephrase the questions.


\paragraph{Implementation Details}
We use open-source Qwen2.5-Coder-7B-Instruct model for experiments. During both training and inference, we adopt database prompts from CodeS~\citep{DBLP:journals/pacmmod/codes}, which provide filtered schema components, values, and metadata, and have demonstrated competitive performance on the BIRD benchmark~\citep{DBLP:conf/nips/bird,Schema_Linking_Knapsack}. We train the model using the GRPO~\citep{GRPO} algorithm within the OpenRLHF~\citep{OpenRLHF} framework. The training is configured with a batch size of 64 and learning rate of 2e-6. In the rollout phase, we sample 8 outputs per input with a temperature $T$ of 1.0, set the maximum sequence length to 4096, and up to maximum interactions $N{=}10$.  The reward function includes five components—format, exact match, execution, entity match, and exploration—each assigned weights of 2.0, 1.0, 3.0, 1.0, and 2.0, respectively. During inference, we apply greedy decoding ($T{=}0.0$), and tree-structured decoding ($T{=}0.7$), allowing up to 3 children per node and generating up to 16 candidates.  We use SQLite~\citep{sqlite} as the SQL executor to obtain execution feedback and apply self-consistency.  All experiments are conducted on a system with a 24-core Intel(R) Xeon(R) Silver 4310 CPU at 2.10GHz, 2048 GB of RAM, and 8 NVIDIA A800 GPUs (80 GB each).









\subsection{Overall Performance Evaluation}
% 展示 bird 和spider 的主要结果，并且展示 spider 变种的结果


\begin{table}[t]
% \centering
\begin{minipage}{0.51\linewidth}
% \centering
\caption{Performance comparison on BIRD and Spider benchmarks (\% Scores).}%标题
\label{table:exp1_indomain}
% \centering%把表居中
\scriptsize % 更小的是\scriptsize，然后是\footnotesize，最小的是 \tiny，然后是\small，再然后是\normalsize，
\setlength{\tabcolsep}{2.2pt}  % 将列间距设为4pt
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{ Methods} & \multicolumn{2}{c}{ BIRD Dev }& \multicolumn{2}{c}{ Spider Dev } & \multicolumn{1}{c}{Spider Test}\\
    \cmidrule(r){2-3} \cmidrule(l){4-5} \cmidrule(l){6-6} 
    & EX  & VES & EX & TS &  EX \\
\midrule
XiYan-SQL~\citep{xiyansql} & \textbf{73.3} & - & - & - & \textbf{89.6} \\
CHASE-SQL + Gemini 1.5~\citep{pourreza2024chase} & 73.0 & \textbf{73.0} & - & - & 87.6 \\
MCTS-SQL + GPT-4~\citep{MCTS-SQL} & 69.4 & 66.2 & 88.7 & - & 86.6 \\
PAS-SQL + GPT-4o~\citep{PAS-SQL} & 64.7 & 65.0 & 87.9 & - & 86.8 \\
MCS-SQL + GPT-4~\citep{mcssql} & 63.4 & 64.8 & \textbf{89.5} & - & \textbf{89.6} \\
MAC-SQL + GPT-4~\citep{DBLP:journals/corr/macsql} & 59.4 & 66.2 & 86.8 & \textbf{82.8} & - \\
DAIL-SQL + GPT-4~\citep{DBLP:journals/pvldb/dail} & 54.8 & 56.1 & 83.5 & 76.2 & - \\
\midrule
SENSE-13B~\citep{DBLP:SENSE} & 55.5 & - & 84.1 & 83.5 & 86.6 \\
DPO + Qwen2.5-Coder-7B~\citep{Dpo-sql} & 64.1 & - & 82.6 & 80.2 & - \\
SFT CodeS-7B~\citep{DBLP:journals/pacmmod/codes} & 57.2 & 58.8 & 85.4 & 80.3 & - \\
OmniSQL-7B~\citep{OmniSQL} & \textbf{66.1} & - & 81.6 & - & \textbf{88.9} \\
DTS-SQL + DeepSeek-7B~\citep{DTS-SQL} & 55.8 & 60.3 & 82.7 & 78.4 & - \\
DB-Explore-7B~\citep{DB-Explore} & 52.1 & 55.8 & 84 & 79.3 & - \\
ROUTE + Qwen2.5-7B~\citep{ROUTE} & 55.9 & 57.4 & 83.6 & 77.5 & 83.7 \\
SQL-o1 + Llama3-8B~\citep{SQL-o1} & 63.4 & 64.7 & 87.4 & 79.6 & 85.4 \\
\midrule
ReEx-SQL-7B (\textbf{Our}) & 64.9 & \textbf{73.1} & \textbf{88.8} & \textbf{83.7} & 86.6 \\
\bottomrule
\end{tabular}
\end{minipage}
\hfil% l
\begin{minipage}{0.44\linewidth}
\centering
\caption{Performance comparison on Spider variants robustness benchmarks (\% Scores).}%标题
\label{table:exp1_outdomain}
\centering%把表居中
\scriptsize % 更小的是\scriptsize，然后是\footnotesize，最小的是 \tiny，然后是\small，再然后是\normalsize，
\setlength{\tabcolsep}{2.2pt}  % 将列间距设为4pt
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{2}{c}{Syn} & \multicolumn{2}{c}{Realistic} & \multicolumn{1}{c}{DK}\\
    \cmidrule(r){2-3} \cmidrule(l){4-5} \cmidrule(l){6-6}
    & EX  & TS  & EX & TS& EX \\
    \midrule
FastRAT\textsubscript{ext}+GPT-4~\citep{fastrat} & 74.4 & - & \textbf{80.9} & - & 72.3 \\
TA-SQL + GPT-4~\citep{TASQL} & - & - & 79.5 & - & 72.9 \\
CYCLESQL + GPT-4~\citep{CYCLESQL} & \textbf{76.0} & \textbf{66.3} & 70.6 & 56.9 & \textbf{68.5} \\
SQL-PaLM + PaLM2~\citep{SQLpalm}  & 74.6 & - & 77.6 & - & 66.5 \\
\midrule
DPO + Qwen2.5-Coder-7B~\citep{Dpo-sql} & 76.2 & - & 79.1 & - & 72.9 \\
Qwen2.5-Coder-32B~\citep{OmniSQL} & 70.5 & - & 74.8 & - & 78.3 \\
ROUTE + Llama3-8B~\citep{ROUTE} & 77.4 & 70.2 & 80.9 & 72.6 & 74.6 \\
SFT CodeS-7B~\citep{DBLP:journals/pacmmod/codes} & 76.9 & 70.0 & 82.9 & 77.2 & 72.0 \\
SFT CodeS-15B~\citep{DBLP:journals/pacmmod/codes} & 77.0 & 69.4 & 83.1 & 75.6 & 70.7 \\
SENSE-7B~\citep{DBLP:SENSE} & 72.6 & 64.9 & 82.7 & 75.6 & 77.9 \\
SENSE-13B~\citep{DBLP:SENSE} & 77.6 & 70.2 & 84.1 & 76.6 & \textbf{80.2} \\
OmniSQL-7B~\citep{OmniSQL} & 69.6 & - & 78.0 & - & 77.8 \\
OmniSQL-14B~\citep{OmniSQL} & 72.0 & - & 78.5 & - & 74.8 \\
OmniSQL-32B~\citep{OmniSQL} & 72.1 & - & 77.2 & - & 77.6 \\
SQL-o1 + Llama3-8B~\citep{SQL-o1} & 77.6 & 69.2 & 82.7 & 72.8 & 78.7 \\
\midrule
ReEx-SQL-7B (\textbf{Our}) & \textbf{78.6} & \textbf{72.1} & \textbf{85.2} & \textbf{79.1} & 79.8 \\
\bottomrule
\end{tabular}
\end{minipage}
\end{table}



\paragraph{Evaluation on In-domain Benchmarks} 
Table~\ref{table:exp1_indomain} presents the performance across the BIRD and Spider benchmarks, highlighting the following: (1) Among models of similar size, it achieves the best EX (88.8\%) and TS (83.7\%) scores on Spider Dev, outperforming all open-source competitors; (2) ReEx-SQL-7B achieves 64.9\% EX on BIRD Dev without data augmentation, close to OmniSQL-7B’s 66.1\%, which relies on extra training data—highlighting ReEx-SQL’s data efficiency. (3) ReEx-SQL-7B outperforms GPT-4/4o-based methods on Spider Dev and achieves the best VES score (73.1\%), despite a gap on BIRD Dev compared to XiYan-SQL (73.3
\%). Overall, ReEx-SQL shows strong superiority without relying on extra data or closed-source models.

\paragraph{Robustness Evaluation}
Table~\ref{table:exp1_outdomain} shows the robustness evaluation across three Spider variants, highlighting the following: (1) ReEx-SQL-7B achieves 78.6\% on Spider-Syn and 85.2\% on Spider-Realistic, outperforming both open and closed models. (2) It also leads in TS scores, with 72.1\% on Spider-Syn and 79.1\% on Spider-Realistic, indicating better structural alignment and lower semantic error. (3) On Spider-DK, ReEx-SQL reaches 79.8\%, just 0.4\% below the 13B model SENSE, despite using fewer parameters and no additional augmented data. Overall, ReEx-SQL-7B demonstrates strong robustness and generalization under various perturbations and knowledge gaps.

\subsection{Training Strategy and Output Format Comparison}

\begin{table}[t]
\caption{Comparison of training strategies and output formats on multiple Text-to-SQL benchmarks. All results are obtained using Qwen2.5-coder-7B with greedy decoding. “Direct Output” denotes directly predicting SQL, “Reason” denotes predicting intermediate reasoning steps before SQL, and “Reason with Execution” further incorporates execution feedback into the reasoning process.}
\label{table:exp2_baseline_and_exec_compare}
\centering%把表居中
\scriptsize %\footnotesize，然后是\footnotesize，最小的是 \tiny，然后是\small，再然后是\normalsize，
\setlength{\tabcolsep}{1.8pt}  % 将列间距设为4pt
\begin{tabular}{ccccccccccc}
\toprule
\multirow{2}{*}{ \makecell{Training \\Type}} & \multirow{2}{*}{\makecell{Output\\ Type}} & \multicolumn{1}{c}{BIRD Dev }& \multicolumn{2}{c}{ Spider Dev } & \multicolumn{1}{c}{Spider Test} & \multicolumn{2}{c}{Spider-Syn} & \multicolumn{2}{c}{Spider-Realistic} & \multicolumn{1}{c}{Spider-DK}\\
    \cmidrule(r){3-3} \cmidrule(r){4-5} \cmidrule(l){6-6} \cmidrule(l){7-8}  \cmidrule(l){9-10}   \cmidrule(l){11-11} 
    & & EX (\%) & EX (\%) & TS (\%) &  EX (\%)  & EX (\%) & TS (\%)  & EX (\%) & TS (\%)  & EX (\%) \\
\midrule
No Post-Training & Direct Output & 48.7 & 81.4 & 75.3 & 79.3 & 68.3 & 54.6 & 77.0 & 68.4 & 71.6 \\
No Post-Training & Standard Reasoning & 49.5 & 81.1 & 74.8 & 78.3 & 69.5 & 56.9 & 74.6 & 63.1 & 71.4 \\
No Post-Training & Execution-Aware Reasoning & 48.6 & 80.0 & 75.9 & 37.0 & 57.4 & 43.1 & 65.7 & 53.8 & 57.6 \\
SFT & Direct Output & 56.3 & 85.4 & 81.4 & 84.5 & 75.7 & 68.3 & 81.9 & 74.2 & 74.0 \\
\midrule
GRPO (Baseline) & Standard Reasoning & 60.8 & 85.7 & 83.5 & 86.2 & 78.3 & 68.9 & 82.3 & 75.6 & 74.6 \\
GRPO (ReEx-SQL) & Execution-Aware Reasoning 
& \textbf{63.4\textsubscript{+2.6}} 
& \textbf{88.4\textsubscript{+2.7}} 
& \textbf{83.5\textsubscript{+0.0}} 
& \textbf{86.4\textsubscript{+0.2}} 
& \textbf{78.5\textsubscript{+0.2}} 
& \textbf{72.1\textsubscript{+3.2}} 
& \textbf{85.0\textsubscript{+2.7}} 
& \textbf{78.7\textsubscript{+3.1}} 
& \textbf{79.3\textsubscript{+4.7}} \\
\bottomrule
\end{tabular}
\end{table}


Table~\ref{table:exp2_baseline_and_exec_compare} compares different training strategies and output formats.  Note that Reason and Reason with Execution are not fine-tuned using SFT due to the additional cost of constructing intermediate reasoning steps. Moreover, ReEx-SQL and the baseline share the same training configuration and reward weights. The baseline does not incorporate exploration, so no exploration reward is used. Highlighting the following: (1) ReEx-SQL consistently outperforms the baseline under GRPO, with EX improvements of +2.6\% on BIRD Dev (63.4\% vs. 60.8\%), +2.7\% on Spider Dev (88.4\% vs. 85.7\%), and +4.7\% on Spider-DK (79.3\% vs. 74.6\%). This confirms that execution feedback improves the model's ability to reason and revise. (2) Without training, Reason with Execution performs worst, especially on BIRD Dev (48.6\%). After GRPO training, it achieves the best result (63.4\%), showing the model learns to generate structured reasoning and SQL effectively. (3) Compared to SFT, GRPO achieves better performance without additional reasoning supervision. For instance, on BIRD Dev, SFT reaches 56.3\%, while all GRPO models exceed 60\%.



\begin{figure}[t]
    \includegraphics[width=1\columnwidth]{figs/compare.pdf} % 替换成你的图像文件名
    \caption{Comparison between the baseline (``Reason'') and ReEx-SQL (``Reason with Execution'') across five aspects. (a) Training reward over steps. (b) Response length across training steps. (c) BIRD performance at different difficulty levels. (d) Distribution of error types on BIRD Dev. (e) Spider performance at different difficulty levels.}
    \label{fig:exp2_baseline_and_exec_compare}
\end{figure}

\paragraph{ReEx-SQL vs. baseline} 
Figure~\ref{fig:exp2_baseline_and_exec_compare} compares ReEx-SQL and the baseline across five aspects, highlighting the following: (1) Training reward (Figure~\ref{fig:exp2_baseline_and_exec_compare}a): Both models converge quickly, but ReEx-SQL consistently achieves higher average rewards throughout training. (2) Reasoning length (Figure~\ref{fig:exp2_baseline_and_exec_compare}b): ReEx-SQL shows a sharp increase in reasoning length at early stages, then quickly stabilizes. In contrast, the baseline only starts increasing after more training steps. (3) Performance on hard examples (Figures~\ref{fig:exp2_baseline_and_exec_compare}c and~\ref{fig:exp2_baseline_and_exec_compare}e): ReEx-SQL significantly outperforms the baseline on complex cases—on BIRD Dev, 49.3\% vs. 43.1\% (+6.2\%);  On Spider Dev, 69.9\% vs. 58.4\% (+11.5\%).  (4) Error analysis (Figure~\ref{fig:exp2_baseline_and_exec_compare}d):  On BIRD Dev, ReEx-SQL reduces total errors from 603 to 562, and syntax errors from 29 (4.5\%) to 11 (1.9\%).  Spider Dev is omitted due to its low syntax error rate. Overall, ReEx-SQL excels in handling complex queries, achieving higher execution accuracy on challenging examples.  It effectively reduces both syntactic and semantic errors, demonstrating more reliable and robust SQL generation.




\subsection{Ablation Study on Reward Design}




\begin{table}[t]
% \centering
\begin{minipage}{0.4\linewidth}
\centering

% \raggedleft
\caption{Ablation of Reward Components on BIRD Dev. ``All Reward'' uses the ``Base'' configuration of reward weights as defined in Table~\ref{table:exp3_reward_weight}.}%标题
\label{table:exp3_reward_wo}
% \centering%把表居中
\scriptsize % 更小的是\scriptsize，然后是\footnotesize，最小的是 \tiny，然后是\small，再然后是\normalsize，
\setlength{\tabcolsep}{2.2pt}  % 将列间距设为4pt
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{Reward Components} & \multicolumn{2}{c}{ BIRD Dev }\\
        \cmidrule(r){2-3}
        & EX (\%) & VES (\%)  \\
\midrule
All Reward & \textbf{60.9} & \textbf{70.8} \\
w/o Exact Match Reward & 58.0 {\tiny (\ensuremath{\downarrow} 2.9)} & 65.4 {\tiny (\ensuremath{\downarrow} 5.4)} \\
w/o Execution Reward & 54.4 {\tiny (\ensuremath{\downarrow} 6.5)} & 62.7 {\tiny (\ensuremath{\downarrow} 8.1)}\\
w/o Entity Match Reward & 57.8 {\tiny (\ensuremath{\downarrow} 3.1)} & 66.1 {\tiny (\ensuremath{\downarrow} 4.7)}\\
w/o Exploration Reward & 59.2 {\tiny (\ensuremath{\downarrow} 1.7)} & 69.3 {\tiny (\ensuremath{\downarrow} 1.5)}\\
\bottomrule
\end{tabular}
\end{minipage}
\hfil% l
\begin{minipage}{0.56\linewidth}
\centering
% \raggedright
% \raggedleft
\caption{Ablation of Reward Weights on BIRD Dev. ``Base'' is the initial setting, ``MaxTune'' is best tuned, others are variants as attempts. EX denotes execution reward; EM denotes exact match reward.}%标题
\label{table:exp3_reward_weight}
\centering%把表居中
\scriptsize % 更小的是\scriptsize，然后是\footnotesize，最小的是 \tiny，然后是\small，再然后是\normalsize，
\setlength{\tabcolsep}{2.2pt}  % 将列间距设为4pt
\begin{tabular}{cccccccc}
\toprule
\multirow{2}{*}{ \makecell{Configuration\\ Type}} &  \multicolumn{5}{c}{Reward Weights} & \multicolumn{2}{c}{ BIRD Dev }\\
\cmidrule(r){2-6} \cmidrule(r){7-8}
 & Format & EM & EX & Entity & Exploration & EX (\%) & VES (\%) \\
\midrule
Base & 1.5 & 0.8 & 1.5 & 0.8 & 0.5 & 60.9 & 70.8 \\
HighExploration & 1.5 & 0.8 & 1.5 & 0.8 & 2.0 & 62.0 & 69.4 \\
HighFormat-EX & 2.0 & 0.8 & 3.0 & 0.8 & 0.5 & 62.3 & 70.1 \\
Uniform & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 62.3 & \textbf{73.8} \\
MaxTune (\textbf{Best}) & 2.0 & 1.0 & 3.0 & 1.0 & 2.0 & \textbf{63.4} & 72.3 \\
\bottomrule
\end{tabular}
\end{minipage}
\end{table}



\paragraph{Impact of Reward Components}
Table~\ref{table:exp3_reward_wo} shows the effect of each reward, highlighting the following: (1) Execution reward has the largest impact (–6.5\% EX), followed by exact match and entity match rewards. (2) Exploration reward has the smallest effect on accuracy (–1.7\% EX), but as shown in Figure~\ref{fig:wo_reward}, it mainly enhances output diversity.

\paragraph{Impact of Reward Weights}
Table~\ref{table:exp3_reward_weight} shows how different reward weight configurations affect ReEx-SQL on BIRD Dev, highlighting the following: (1) Increasing exploration reward (HighExploration) improves EX (60.9\% → 62.0\%), suggesting that encouraging diverse reasoning paths helps execution accuracy. (2) Emphasizing format and execution rewards (HighFormat-EX) further improves EX to 62.3\%, confirming their importance in guiding logical generation.  (4) MaxTune, which boosts format, execution, and exploration simultaneously, yields the best overall performance (EX 63.4\%), highlighting the synergistic effect of combining multiple reward signals.  Appendix~\ref{app:reward_design} presents reward trends, reasoning length, and exploration counts under different component and weight configurations.





\subsection{Decoding Strategy Comparison}




\begin{table}[t]
\caption{Comparison of Decoding Strategies on BIRD and Spider Benchmarks. Tree-based decoding achieves superior efficiency and competitive accuracy compared to other sampling methods.}
\label{table:exp4_comparsion_decoding}
\centering%把表居中
\footnotesize %\scriptsize，然后是\footnotesize，最小的是 \tiny，然后是\small，再然后是\normalsize，
\setlength{\tabcolsep}{3.2pt}  % 将列间距设为4pt
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{Decoding Strategy} & \multicolumn{3}{c}{BIRD Dev}  & \multicolumn{3}{c}{ Spider Dev} \\
\cmidrule(r){2-4} \cmidrule(r){5-7}
 & EX(\%) & VES(\%) & Time (s/sample) \ensuremath{\downarrow} & EX(\%) & TS(\%) & Time (s/sample) \ensuremath{\downarrow} \\
\midrule
Greedy Decoding & 63.4 & 72.7 & 0.6 & 88.4 & 83.5 & 0.2 \\
\midrule
8-Sampling & 64.1 & \textbf{72.7} & 2.8 & 88.3 & 83.6 & 1.4 \\
Tree-Based Decoding (Max 8)  & \textbf{64.2} & 72.2 & \textbf{2.0 {\scriptsize (\ensuremath{\downarrow} 28.6\%)}} & \textbf{88.4} & \textbf{83.6} & \textbf{0.9 {\scriptsize (\ensuremath{\downarrow} 35.7\%)}} \\
\midrule
16-Sampling & 64.5 & 72.9 & 5.4 & 88.5 & 83.5 & 2.8 \\
Tree-Based Decoding (Max 16) & \textbf{64.9} & \textbf{73.1} & \textbf{2.6 {\scriptsize (\ensuremath{\downarrow} 51.9\%)}} & \textbf{88.8} & \textbf{83.7} & \textbf{1.1 {\scriptsize (\ensuremath{\downarrow} 60.7\%)}} \\
\bottomrule
\end{tabular}
\end{table}



Table~\ref{table:exp4_comparsion_decoding} compares the performance of different decoding strategies for ReEx-SQL, highlighting the following: (1) Tree-Based Decoding significantly enhances efficiency for single-sample decoding under the 16-candidate setting, reducing time by 60.7\% on the Spider dataset (2.8s → 1.1s) and 51.9\% on the BIRD dataset (5.4s → 2.6s), while maintaining or surpassing accuracy. (2) Tree-Based Decoding slightly outperforms Sampling in accuracy, demonstrating its ability to achieve both high efficiency and strong generation quality.


\subsection{Impact of Execution Feedback and Database}

\begin{table}[t]
\caption{Impact of Execution Feedback and Database Complexity on ReEx-SQL.  ``Origin'' denotes the original databases of BIRD and Spider benchmarks, while ``TS'' refers to the TS database~\citep{Test-Suites}, which is only applicable to Spider and its variants and augments them with additional database values. ``Nums'' indicates the maximum number of rows returned by each SQL execution. }
\label{table:exp5_execution_database_impact}
\centering%把表居中
\scriptsize %\footnotesize，然后是\footnotesize，最小的是 \tiny，然后是\small，再然后是\normalsize，
\setlength{\tabcolsep}{3.2pt}  % 将列间距设为4pt
\begin{tabular}{cccccc|ccccc|ccccc}
\toprule
\multirow{2}{*}{Database} & \multirow{2}{*}{Nums} & \multicolumn{4}{c}{BIRD Dev (EX\%) }& \multicolumn{5}{c}{ Spider Test (EX\%)} & \multicolumn{5}{c}{Spider-DK (EX\%)} \\
\cmidrule(r){3-6} \cmidrule(r){7-11} \cmidrule(r){12-16} 
 &  & Simple & Moderate & Challenging & Total & Easy & Medium & Hard & Extra & All & Easy & Medium & Hard & Extra & All \\
\midrule
Origin & 3 & \textbf{69.5} & 55.5 & 49.3 & 63.4 & 93.8 & 89.0 & 82.1 & 76.2 & 86.4 & 88.2 & 85.4 & 62.2 & 67.6 & 79.3 \\
Origin & 6 & 69.4 & 55.7 & 49.3 & 63.4 & \textbf{94.0} & 89.0 & 82.3 & \textbf{76.5} & 86.6 & 88.2 & 85.8 & 64.9 & 66.7 & 79.6 \\
Origin & 8 & 69.4 & \textbf{55.9} & \textbf{50.0} & \textbf{63.5} & 93.8 & 89.0 & 82.3 & 76.2 & 86.5 & 88.2 & 85.8 & 64.9 & \textbf{67.8} & 79.8 \\
\midrule
TS & 3 & - & - & - & - & \textbf{94.0} & 89.0 & \textbf{82.7} & \textbf{76.5} & \textbf{86.7 }& 88.2 & \textbf{86.2} & 64.9 & 67.6 & \textbf{80.0} \\

\bottomrule
\end{tabular}
\end{table}




Table~\ref{table:exp5_execution_database_impact} examines the impact of execution feedback (maximum returned rows, Nums) and database content (Original vs. TS) on ReEx-SQL performance. Key findings are as follows:
(1) Execution Feedback: Increasing returned rows slightly improves performance, e.g., Nums from 3 to 8 boosts BIRD Challenging by 0.7\% (49.3\% → 50.0\%), indicating that richer feedback helps the model better assess result correctness. (2) Compared to the original database, TS databases with additional cell values further improve performance, e.g., Spider Test Hard by 0.6\% (82.1\% → 82.7\%) and Spider-DK to 80.0\% (79.3\% → 80.0\%). Overall, richer execution signals and enhanced databases positively affect generation quality.



